"Let Your Characters Tell Their Story": A Dataset for Character-Centric Narrative Understanding

When reading a literary piece, readers often make inferences about various characters' roles, personalities, relationships, intents, actions, etc. While humans can readily draw upon their past experiences to build such a character-centric view of the narrative, understanding characters in narratives can be a challenging task for machines. To encourage research in this field of character-centric narrative understanding, we present LiSCU -- a new dataset of literary pieces and their summaries paired with descriptions of characters that appear in them. We also introduce two new tasks on LiSCU: Character Identification and Character Description Generation. Our experiments with several pre-trained language models adapted for these tasks demonstrate that there is a need for better models of narrative comprehension.

==> 5-results.tex <==




% \begin{table}[t]
% \scriptsize
%     \centering
%     \input{figures/discriminative_res}
%     \caption{Accuracy and MRR for the discriminative task.}
%     \label{tab:disc-res}
% \end{table}

% \setlength\tabcolsep{4pt}
%     \begin{tabular}{lllll}
%     \toprule
%     \textbf{Model} & \textbf{Ppl.} & \textbf{BLEU-4} & \textbf{ROUGE-L} & \textbf{Human Eval.} \\ 
%     \midrule
%     GPT2-XL & ??? & ??? & ??? & ??? \\ 
%     BART-L & ??? & ??? & ??? & ??? \\ 
%     \bottomrule
%     \end{tabular}
% \setlength\tabcolsep{6pt}

% \setlength\tabcolsep{2pt}
%     \begin{tabular}{llll p{0.01cm} llll}
%     \toprule
%     \textbf{Objective} & \textbf{Model} & \multicolumn{2}{c}{\textbf{Automatic}} & & \multicolumn{4}{c}{\textbf{Human (\%)}} \\ 
%     \hhline{~~--~----}
%     & & \textbf{BLEU} & \textbf{ROUGE} & & \textbf{Gram.} & \textbf{Rele.} & \textbf{Corr.} & \textbf{Expl.} \\ 
%     \midrule
%     \rowcolor{blue!10} \multicolumn{9}{c}{\textbf{Post-hoc Rationalization}} \\
%     % \midrule
%     \multirow{2}{*}{\textbf{Rationale}} & GPT2-XL & 33.0 & 33.91 & & 92.5/93.5 & 33.5/60 & 52.5/45.5 & 2.0/4.5 \\ 
%     & BART-L & 13.15 & 22.48 & &  \textbf{95/99.5} & \textbf{80/80.5} & \textbf{55/58} & \textbf{47/33} \\ 
%     \midrule
%     \multirow{2}{*}{\textbf{Multi}} & GPT2-XL & \textbf{33.58} & \textbf{34.50} & & 88.5/94.5 & 30/55 & 47/43 & 0.5/7.0 \\ 
%     & BART-L & 17.38 & 24.03 & & 95/97.5 & 74.5/76.5 & 55.5/53 & 44/22.5 \\    
%     \midrule
%     \rowcolor{blue!10} \multicolumn{9}{c}{\textbf{Joint Prediction and Rationalization}} \\
%     % \midrule
%     \textbf{Update} & GPT2-XL & 23.93 & \textbf{31.71} & & 85/88 & 15.5/35 & 30.5/15.5 & 1.0/1.5 \\ 
%     \textbf{+ Rationale} & BART-L & 25.24 & 30.83 & & 86.5/83 & 20/34.5 & 34/17.5 & 2.5/0.5 \\    
%     \midrule
%     \textbf{Update type} & GPT2-XL & \textbf{27.90} & 31.18 & & 86.5/85.5 & \textbf{27/39} & \textbf{36.5/29} & \textbf{8.5/3.0} \\ 
%     \textbf{+ Rationale} & BART-L & 24.54 & 29.04 & & 86.5/85.5 & 26/18.5 & 35.5/30.5 & 7.0/1.0 \\    
%     \bottomrule
%     \end{tabular}
% \setlength\tabcolsep{6pt}

==> figures/results-fine.tex <==
% fine-grained results based on fact coverage
\setlength\tabcolsep{3.3pt}
    \renewcommand{\arraystretch}{1.4}
    \begin{tabular}{lc p{0.001cm} ccc p{0.001cm} c}
    \toprule
    % \textbf{Objective} & \textbf{Model} & \multicolumn{2}{c}{\textbf{Automatic}} & & \multicolumn{4}{c}{\textbf{Human (\%)}} \\ 
    % \hhline{~~--~----}
    \textbf{Model} & \textbf{BLEU} && \textbf{ROUGE-1} & \textbf{ROUGE-2} & \textbf{ROUGE-L} & & \textbf{BERT-F1} \\ 
    \midrule
    \rowcolor{blue!10} \multicolumn{8}{c}{\textbf{Length Truncated Input}} \\
    % \midrule
    \textbf{GPT2-L} & 0.90/0.71/0.60/0.59/0.48 & & 20.33/19.94/18.81/19.39/16.90 & 4.34/3.60/3.36/3.32/2.65 & 18.50/17.91/17.14/17.84/14.82 & & 76.23/80.11/76.53/75.81/83.05 \\ 
    \textbf{BART-L} & \textbf{2.31/1.60/1.11/0.98/0.91}  & & \textbf{27.04/25.83/23.77/24.31/22.53} & \textbf{7.10/5.86/5.14/4.77/4.35} & \textbf{23.83/22.98/21.08/21.34/19.87} & & 85.30/85.00/84.34/84.14/83.67 \\
    \textbf{Longformer} & 1.86/1.06/0.92/0.70/0.47 & & 24.16/21.78/20.55/20.20/19.22 & 6.80/4.62/4.33/3.98/3.92 & 22.05/19.65/18.71/18.26/16.63 & & 85.60/84.92/84.46/84.24/83.89 \\
    % \multirow{2}{*}{\textbf{Rationale}} & GPT2-XL & 33.0 & 33.91 & & 92.5/93.5 & 33.5/60 \\ 
    % & BART-L & 13.15 & 22.48 & &  \textbf{95/99.5} & \textbf{80/80.5} \\ 
    % \midrule
    % \multirow{2}{*}{\textbf{Multi}} & GPT2-XL & \textbf{33.58} & \textbf{34.50} & & 88.5/94.5 & 30/55  \\ 
    % & BART-L & 17.38 & 24.03 & & 95/97.5 & 74.5/76.5 \\    
    \midrule
    \rowcolor{blue!10} \multicolumn{8}{c}{\textbf{Coreference Truncated Input}} \\
    % \midrule
    \textbf{GPT2-L} & 0.82/0.63/0.53/0.58/0.37 & & 19.80/19.24/17.96/18.49/16.77 & 3.86/3.24/3.06/3.04/2.16 & 17.79/17.39/16.46/16.62/16.27 & & 76.16/79.52/78.33/80.23/68.71 \\ 
    \textbf{BART-L} & 1.98/1.05/0.79/0.54/0.48 & & 23.81/22.30/20.69/19.30/17.81 & 6.46/4.90/4.43/3.71/3.48 & 21.28/20.03/18.33/17.29/16.27 & & 85.09/84.78/84.14/83.81/83.20\\
    \textbf{Longformer} & 1.78/1.09/0.77/0.65/0.60 & & 23.32/22.23/20.23/19.90/18.61 & 6.04/4.80/3.96/3.57/3.57 & 21.41/20.22/18.16/17.70/16.81 & & 85.43/85.07/84.47/84.12/83.65\\
    \midrule
    \rowcolor{blue!10} \multicolumn{8}{c}{\textbf{Full Length Input}} \\
    \textbf{Longformer} & 2.15/1.31/1.04/0.65/0.55 & & 24.47/22.56/20.90/20.63/19.90 & 6.98/5.37/4.63/3.84/3.48 & 21.91/20.40/18.85/18.48/17.73 & & \textbf{85.66/85.11/84.57/84.35/83.97} \\
    \bottomrule
    \end{tabular}
\setlength\tabcolsep{6pt}

==> other_contents.tex <==
 
 Joshua Maynez et al. 2020: A model with a poorly- informed decoder and that is agnostic to the divergence issue between the source and target texts (Wiseman et al., 2017; Dhingra et al., 2019), will function more as an open-ended language model and will be prone to extrinsic hallucinations.
 
 Section 2.2:  A model with a poorly- informed decoder and that is agnostic to the di- vergence issue between the source and target texts (Wiseman et al., 2017; Dhingra et al., 2019), will function more as an open-ended language model and will be prone to extrinsic hallucinations.
 
 
 In this paper we stand in favour of the assertion that abstractive systems may integrate with the background knowledge to generate rich and mean- ingful summaries. More concretely, \textbf{“hallucinations in summarization are acceptable if they lead to better summaries that are factual with respect to the document and the associated background knowledge.”} This assumption also allows us to assess the capability of recent neural models to integrate with the background knowledge to generate factual abstracts (see Section 5.3).
 
 
 However, the percentage of system summaries with intrinsic hallucination was much higher than in gold summaries (7.4\% vs others). This phenomenon particularly revealed the models’ tendency to misrepresent information in the document due to the lack of document-level understanding and inference. 
 
 It appears that BERTS2S is overall most conservative among all four abstractive systems while getting closer to reference summaries in terms of ROUGE. The pre- training prepares BertS2S to be more aware of the domain of the document and less prone to language model vulnerabilities. Consequently, BertS2S is more confident in predicting tokens from the docu- ment than TranS2S, hence, improving faithfulness.
 
 NOTE TO ME: probably mention that pre-training models have access to large amount of story like data which gives them some prior knowledge helping then to generate better description compared to models radinly initialized from scratch.
